Cross Entropy Hyperparameter Optimization for Constrained Problem Hamiltonians Applied to QAOA

Hybrid quantum-classical algorithms such as the Quantum Approximate Optimization Algorithm (QAOA) are considered as one of the most encouraging approaches for taking advantage of near-term quantum computers in practical applications. Such algorithms are usually implemented in a variational form, combining a classical optimization method with a quantum machine to find good solutions to an optimization problem. The solution quality of QAOA depends to a high degree on the parameters chosen by the classical optimizer at each iteration. However, the solution landscape of those parameters is highly multi-dimensional and contains many low-quality local optima. In this study we apply a Cross-Entropy method to shape this landscape, which allows the classical optimizer to find better parameter more easily and hence results in an improved performance. We empirically demonstrate that this approach can reach a significant better solution quality for the Knapsack Problem.

==> alternative_qaoa_section.tex <==
The variational form of QAOA first starts from a uniform superposition state of every possible solution. This is done by applying Hadamard gates to each qubit. Subsequently an alternating sequence of operators of length $p$ evolves the system. 
For $p=2$, two unitary operators are used to describe this evolution:

\begin{equation*}U = U(H_{p_1})U(H_{p_0})\end{equation*} 

Each $U(H_{p_i})$ is approximated by a first order Suzuki-Trotter decomposition with the number of Trotter steps equal to one
\begin{equation*}U(H_{p_i}) = U(H_D,\beta_i)U(H_C,\gamma_i) \end{equation*} 
where ${U(H_C,\gamma_i) = exp(-i\gamma_iH_C)}$ and ${U(H_D,\beta_i) = exp(-i\beta_iH_D)}$.

Here $H_D = \frac{1}{2} \sum_{i} \sigma^X_i$ is the so called driver Hamiltonian with $\sigma^X$ being the Pauli X-operator \begin{equation*}\sigma^X = \begin{pmatrix} 0 & 1 \\ 1 & 0  \end{pmatrix}\end{equation*}. $\beta_i$ and $\gamma_i$ are angles for the rotation. 


Repeated applications of the cost and driver dynamics evolves the system to the quantum state
\begin{equation}\label{eq:evolve}
\ket{\beta,\gamma} = U(H_D,\beta_i) U(H_C,\gamma_i) ... U(H_D,\beta_1) U(H_C,\gamma_1) U(H_D,\beta_0) U(H_C,\gamma_0)\ket{\psi}.
\end{equation}
